Text-based RL Agents with Commonsense Knowledge: New Challenges, Environments and Baselines

Text-based games have emerged as an important test-bed for Reinforcement Learning (RL) research, requiring RL agents to combine grounded language understanding with sequential decision making. In this paper, we examine the problem of infusing RL agents with commonsense knowledge. Such knowledge would allow agents to efficiently act in the world by pruning out implausible actions, and to perform look-ahead planning to determine how current actions might affect future world states. We design a new text-based gaming environment called TextWorld Commonsense (TWC) for training and evaluating RL agents with a specific kind of commonsense knowledge about objects, their attributes, and affordances. We also introduce several baseline RL agents which track the sequential context and dynamically retrieve the relevant commonsense knowledge from ConceptNet. We show that agents which incorporate commonsense knowledge in TWC perform better, while acting more efficiently. We conduct user-studies to estimate human performance on TWC and show that there is ample room for future improvement.

==> intro_old.tex <==
\section{Introduction}\label{sec:intro}
Over the years, simulation environments and games have been used extensively to showcase and drive advances in reinforcement learning technology. A recent environment that has received much focus is TextWorld (TW)~\cite{cote18textworld}, where an agent must interact with an external environment to achieve goals while maximizing reward - all of this using only the modality of text. TextWorld and similar text-based environments seek to bring advances in language understanding and grounding in a reinforcement (sequential decision making) setting.

\mrinmaya{For the below paragraph, I would suggest instead talking about why RL agents should have commonsense and how commonsense knowledge can make RL more efficient citing Figure 1}

A common thread inherent in solutions to some of the NLP tasks is that mere text-based techniques cannot achieve or beat the human-level performance and that NLP systems must instead learn how to utilize additional knowledge from external sources such as knowledge bases (KBs) and knowledge graphs (KGs) to improve their overall performance. Figure~\ref{fig:kitchen_cleanup} presents a running example that illustrates this: in the figure, the additional knowledge that must be utilized effectively by the agent is presented in the bottom left corner under the {\em ConceptNet} heading.

\mrinmaya{This para is not needed}
In general, the use of external knowledge to improve the accuracy of NLP tasks has garnered significant attention from the community. Specifically, for tasks like natural language inference (NLI), recent work~\cite{kapanipathi2020infusing,wang2019improving} has shown that while external knowledge can bring in useful information, this must be balanced by the context-specific relevance of the new information fed into the system. If this is not done properly, there is a very high risk of overwhelming the agent/algorithm with too much information, leading to poor decisions and performance.

\begin{figure*}[tp]
    \centering
    \includegraphics[width=0.8\linewidth]{img/kitchen_cleanup_new.pdf}
    \caption{{\bf WE NEED TO CHANGE THIS FIGURE TO EXPLAIN OUR NEW ENVIRONMENT.} An illustration of our Kitchen Cleanup game. The agent perceives the world via text and has been given the goal of cleaning up the kitchen. As shown here, the agent can leverage commonsense knowledge from ConceptNet to reduce the exploration and achieve the goal.}
    \label{fig:kitchen_cleanup}
\end{figure*}

\mrinmaya{Now talk about our environments, how were they designed. Our investigation of commmonsense is specific: only about objects, their attributes and affordances}

In this paper, we present a novel approach to the use of external knowledge from the ConceptNet~\cite{liu2004conceptnet,speer2017conceptnet} knowledge graph to reduce the exploration space for a Reinforcement Learning (RL) agent. Specifically, we consider an RL based agent that is able to model the world around it at two levels -- a {\em local}, or {\em belief}, graph that describes its current belief of the state of the world; and a {\em global} or {\em commonsense} graph of entities that are related to that state -- and the interaction between those two levels. 
The belief graph provides the agent with a symbolic way to represent its current perception of the world, which can be easily combined with symbolic commonsense knowledge from the commonsense graph. This two-level representation of the world and the knowledge about it follows the model proposed in the Graph Aided Transformer Agent (GATA)~\cite{adhikari2020learning} framework. 

Using this model, we are able to show a significant improvement in the performance of an RL agent in a kitchen cleanup task that is set in the TextWorld setting. An example of such a kitchen cleanup task is shown in Figure~\ref{fig:kitchen_cleanup}: the agent is given an initial observation (which is used to produce the first iteration of the agent's belief graph), with the final goal of cleaning up the kitchen. The agent has to produce the list of actions that are necessary to achieve this goal: that list is given on the right hand side. Finally, the additional external knowledge from the ConceptNet knowledge graph -- which makes up the global graph for our agent -- is shown at the bottom left. In the case of this running example, the agent may discover from ConceptNet that apples are usually located in refrigerators, and plates are located in cabinets. We will use this kitchen cleanup instance as a running example throughout the paper.

By evaluating our approach on two different tasks -- a {\em kitchen cleanup} task as above, and an additional {\em cooking recipe} task -- we can show that the interaction between the belief and commonsense graphs can reduce the exploration of the RL agent in comparison to the purely text-based model. However, we are also able to demonstrate a more nuanced point: merely providing an agent with commonsense knowledge is not sufficient to improve its performance. Indeed, oftentimes it is detrimental to the agent's performance. We show that this is due to the agent being overwhelmed with too much commonsense knowledge, and discuss how different tasks and settings have different demands on the knowledge that is used by an agent.

Contributions for the dataset paper:
\begin{itemize}
\item Dataset generation 
    \begin{itemize}
        \item Code
        \item Manual effort to create the framework (commonsense cleanup task) -- done
        \item Inter-annotator agreement and analysis -- done
    \end{itemize}
\item Baselines
    \begin{item}
    \item Random
    \item Simple Agent
    \item Knowledge-Aware agent with combinations of local and world graph
    \end{item}
\item Analysis and Claims
    \begin{itemize}
        \item Dataset -- We have X objects, Y rooms mapped with commonsense manually. Inter-annotator agreement. Percentage of links missed vs coverage. (Karthik)
        \item World graph can improve exploration -- Knowledge-Aware agent performs better than both Simple and Random agent. -- Experiments has to be done. -- Run experiments only on World graph with only text-world graph co-attention. 
        \item Simple variations of reducing noise ConceptNet -- 1 Hop, Path based, Filter Path based Manually to provide the ground truth (Relationships as a feature).  Future work -- Better denoising for using commonsense knowledge graphs for RL Agents.
        \item Hardness of the environments -- Increasing number of objects and performance of the knowledge-aware agent. 
        \item Generalizing to a new domain where the train entities and test entities are different -- Last set experiment if we have time.
    \end{itemize}
   
 \textbf{Remarks:} Run the above experiments ``without local graph'' on easy and Medium 1.
 If we are done early (Claim: common sense knowledge is useful along with belief/planning graph): Combining local and world graph -- Not related to the dataset paper -- Combination of multiple rooms vs multiple objects will help to make claims. -- Hard and Medium 2
 
 \item Experiments
    \begin{item}
    \item[Mattia] Easy - random, simple, local, world, local+world (3 runs)
    \item[Keerti]
    \item[Pushkar] 
    \end{item}
\item Future Challenges 
    \begin{itemize}
        \item Denoising the knowledge graph
        \item 
    \end{itemize}
\end{itemize}


% % In this paper, we present the first true use of knowledge-based embeddings from open knowledge sources like ConceptNet in order to improve the performance of a reinforcement learning agent.


% \begin{itemize}
% \item Novel approach to use external knowledge to reduce exploration for an RL Agent. We demostrate the impact of it on Text-World setting.
% \item First one to look at the interaction between Local and Global graphs (GATA paper) and their interaction
% \item We show that the use of external knowledge, in particular the interaction between local and global graphs, reduces the exploration of the RL agent by X\% in comparison to the pure text based.
% \end{itemize}
